Strong size evolution of disc galaxies since z = 1: Readdressing galaxy growth using a physically motivated size indicator

Our understanding of how the size of galaxies has evolved over cosmic time is based on the use of the half-light (effective) radius as a size indicator. Although the half-light radius has many advantages for structurally parameterising galaxies, it does not provide a measure of the global extent of the objects, but only an indication of the size of the region containing the innermost 50% of the galaxy's light. Therefore, the observed mild evolution of the effective radius of disc galaxies with cosmic time is conditioned by the evolution of the central part of the galaxies rather than by the evolutionary properties of the whole structure. Expanding on the works by Trujillo et al. (2020) and Chamba et al. (2022), we study the size evolution of disc galaxies using as a size indicator the radial location of the gas density threshold for star formation. As a proxy to evaluate this quantity, we use the radial position of the truncation (edge) in the stellar surface mass density profiles of galaxies. To conduct this task, we have selected 1048 disc galaxies with M$_{\rm stellar}$ $>$ 10$^{10}$ M$_{\odot}$ and spectroscopic redshifts up to z=1 within the HST CANDELS fields. We have derived their surface brightness, colour and stellar mass density profiles. Using the new size indicator, the observed scatter of the size-mass relation (~0.1 dex) decreases by a factor of ~2 compared to that using the effective radius. At a fixed stellar mass, Milky Way-like (M$_{\rm stellar}$ ~ 5$\times$10$^{10}$ M$_{\odot}$) disc galaxies have on average increased their sizes by a factor of two in the last 8 Gyr, while the surface stellar mass density at the edge position has decreased by more than an order of magnitude from ~13 M$_{\odot}$/pc$^2$ (z=1) to ~1 M$_{\odot}$/pc$^2$ (z=0). These results reflect a dramatic evolution of the outer part of MW-like disc galaxies, growing ~1.5 kpc Gyr$^{-1}$.

==> tables/table_fits_old.tex <==
\begin{table*}
\label{tab:trunc_fits}
\caption{Truncation-related least squares fits with the analytical form $\rm a+bx$ (the subscript R stands for R$_{\rm edge}$ and $\rm \Sigma$ for $\Sigma_{\rm edge}$ respectively)}
\begin{tabular}{ccccccccccc}
\hline \hline
z & b$_{\rm R}$ & a$_{\rm R,b}$ & b$_{\Sigma}$ & a$_{\rm \Sigma,b}$ & \sigma$_{\rm R}$ & \sigma$_{\rm \Sigma}$ & \sigma$_{\rm R,mass}$ & \sigma$_{\Sigma,mass}$ & \sigma$_{\rm R,int}$ & \sigma$_{\rm \Sigma,int}$ \\
\hline
Chamba et al. ($z\sim0.1$) & 0.34 $\pm$ 0.02 & -2.26 $\pm$ 0.01 & 0.32 $\pm$ 0.06 & -3.36 $\pm$ 0.02 & 0.10 & 0.27 & - & - & - & - \\
0.1$< \rm z <$0.3 & 0.34 $\pm$ 0.02 & -2.35 $\pm$ 0.02 & 0.32 $\pm$ 0.06 & -2.98 $\pm$ 0.06 & 0.11 & 0.36 & 0.05 & 0.04 & 0.10 & 0.36 \\
0.3$< \rm z <$0.5 & 0.34 $\pm$ 0.02 & -2.40 $\pm$ 0.01 & 0.32 $\pm$ 0.06 & -2.79 $\pm$ 0.04 & 0.10 & 0.34 & 0.05 & 0.04 & 0.09 & 0.33 \\
0.5$< \rm z <$0.7 & 0.34 $\pm$ 0.02 & -2.47 $\pm$ 0.01 & 0.32 $\pm$ 0.06 & -2.51 $\pm$ 0.03 & 0.12 & 0.35 & 0.05 & 0.04 & 0.10 & 0.35 \\
0.7$< \rm z <$0.9 & 0.34 $\pm$ 0.02 & -2.50 $\pm$ 0.01 & 0.32 $\pm$ 0.06 & -2.37 $\pm$ 0.02 & 0.11 & 0.29 & 0.05 & 0.04 & 0.10 & 0.29 \\
0.9$< \rm z <$1.1 & 0.34 $\pm$ 0.02 & -2.55 $\pm$ 0.01 & 0.32 $\pm$ 0.06 & -2.26 $\pm$ 0.04 & 0.13 & 0.38 & 0.06 & 0.04 & 0.12 & 0.38 \\
\hline
\end{tabular}
\end{table*}

